ImpRAG: Retrieval-Augmented Generation with Implicit Queries

Retrieval-Augmented Generation (RAG) systems traditionally treat retrieval and generation as separate processes, requiring explicit textual queries to connect them. This separation can limit the ability of models to generalize across diverse tasks. In this work, we propose a query-free RAG system, named ImpRAG, which integrates retrieval and generation into a unified model. ImpRAG allows models to implicitly express their information needs, eliminating the need for human-specified queries. By dividing pretrained decoder-only language models into specialized layer groups, ImpRAG optimizes retrieval and generation tasks simultaneously. Our approach employs a two-stage inference process, using the same model parameters and forward pass for both retrieval and generation, thereby minimizing the disparity between retrievers and language models. Experiments on 8 knowledge-intensive tasks demonstrate that ImpRAG achieves 3.6-11.5 improvements in exact match scores on unseen tasks with diverse formats, highlighting its effectiveness in enabling models to articulate their own information needs and generalize across tasks. Our analysis underscores the importance of balancing retrieval and generation parameters and leveraging generation perplexities as retrieval training objectives for enhanced performance.

==> sections/intro.tex <==
\section{Introduction}

\scott{
The current introduction is fine, but I feel that it doesn't highlight the unique problem setting (i.e., query free) enough.
Suggested flow:
\begin{itemize}
    \item What RAG is at high-level? (e.g., having a retriever to bring in tail-knowledge, updated information at inference time)
    \item Although vanilla RAG (basically REPLUG) is mostly used due to its simplicity, joint training Retriever and LM enables the LM to better leverage retrieved results and the Retriever to provide more helpful context. (Can cite many papers here, like REALM, RAG, Atlas, RA-DIT, etc.)
    \item Issues of the joint training methods: query formulation \& separate query embedding. Discuss the negative implications of these two issues.
    \item Describe our solution and explain (1) how it addresses these two issues, and (2) why it's better
    \item What are the technical challenges of our approach, briefly describe them and explain how we overcome those challenges.
    \item Brag about the empirical results
\end{itemize}
}

Retrieval-Augmented Generation (RAG) generally adheres to the \textit{retrieve-then-generate} paradigm \citep{NEURIPS2020_6b493230}. This involves first retrieving the most relevant passages from a retrieval corpus and then incorporating them into the context for large language models (LLMs) to process. While effective, models using this paradigm often treat retrieval and generation as distinct processes, usually requiring separate input templates. This separation can lead to a mismatch between what LLMs need and what retrievers assume is necessary. More importantly, it also limits the models' capacity to fully utilize training supervision from both retrieval and generation, thereby restricting their ability to generalize across different tasks.

In this work, we introduce \thiswork, a novel approach that integrates retrieval and generation into a unified model and process, enabling retrieval using continuous vectors and allowing models to benefit from supervision in both retrieval and generation tasks.\footnote{While retrieval is typically performed by computing vector similarities, previous work has mostly relied on explicitly defined textual queries. In contrast, \thiswork enables the direct retrieval of passages using continuous, implicit queries generated directly by LLMs themselves. Doing so eliminates the need for a separate process or model dedicated to retrieval.\vic{Put this back to the main text? Usually better to not use footnote in the Intro section because it interrupts the flow}} At its core, \thiswork aims to enable retrieval capabilities through retrieval heads in self-attention. Building upon pretrained decoder-only language models, \thiswork divides the layers into three groups: the bottom group for retrieval and the middle and top groups for reading and generation.\vic{\citep{jiang-etal-2022-retrieval} seems very relevant. Maybe give a short summary of prior work on joint retrieve-and-generate, then introduce the proposed method?} To reduce memory costs, we disable attention to retrieved passages in the top layers.
% \mingda{Updated the text here to match the ``three layer groups'' definition used in the main text.}


\begin{figure}[t]
\begin{center}
    \includegraphics[scale=0.38]{figures/inference_diagram.pdf}
    \caption{Diagram illustrating the inference process of \thiswork on the entity linking task. We divide decoder-only LLMs into three layer groups for specialized finetuning: bottom (green), middle (red), and top (blue). The bottom layers are optimized for retrieval tasks. The middle and top layers handle the reading of retrieved passages, with cross-attention disabled in the top layers to reduce memory consumption. \thiswork employs the same input and forward pass for both retrieval and generation, reducing the gap between these processes and allowing models to generalize across tasks with varied formats.\vic{Maybe make this into a larger figure spreading two columns and also illustrate the text in the passages and query?}
    % \wenzheng{Passage embeddings here look weird since the cross attention attend to the key value states and passage embeddings are for retrieval?}\mingda{Good Catch! What about the updated figure?}\wenzheng{Looks great!}
    }\label{fig:arch}
\end{center}
\end{figure}

Figure~\ref{fig:arch} illustrates an example of applying \thiswork to the entity linking task, where models are tasked with linking the mention "British" to an entity in Wikipedia, given the context paragraph. A typical RAG model would require the design of a separate query template, such as using only the mention text, to achieve reasonable retrieval performance. In contrast, \thiswork can perform retrieval and generation jointly without the need for additional template design, making it more generalizable.

During training, we optimize two objectives simultaneously: generation loss and retrieval loss. The generation loss is the standard causal language modeling loss, while the retrieval loss first utilizes pseudo labels generated by trained retrievers to warm up the retrieval ability and then self-improves using its own generation log likelihood for the remainder of the training.



At inference time, we employ a two-stage process. First, we embed passages using the bottom layer for retrieval, and then utilize the top layer group to read the retrieved passages and generate the final responses. By leveraging the same forward pass and model parameters for both retrieval and generation, \thiswork reduces the disparity between retrievers and LLMs.


In experiments, we train models on datasets that either require retrieval or do not. The datasets requiring retrieval are used to enhance retrieval performance, while those not requiring retrieval are used to improve cross-task instruction-following capabilities. We evaluate the models on 8 knowledge-intensive tasks, focusing on different aspects: basic question answering, multihop reasoning, and instruction following. We also establish strong baselines that perform RAG in the retrieve-then-generate paradigm, including % \radit
RA-DIT~\citep{lin2024radit}, a method that iteratively updates LLMs and retrievers to better align the two. Our experiments show that \thiswork performs competitively on tasks with formats similar to the training tasks, without requiring additional inference computations or model parameters. Furthermore, it significantly surpasses previous approaches on instruction-following tasks with more varied formats, removing the necessity to design separate templates for retrieval and generation. This underscores the effectiveness of jointly performing retrieval and generation for RAG.

\todo{Finish the Intro after the results are complete}

\vic{
\begin{enumerate}
    \item The intro hasn't explain what ``query-free'' means despite it's a keyword in the title. I remember we started from this motivation but the theme of the project seems to have evolved into building ``a RAG model using the LLM architecture alone without using an external retriever''. Maybe we can emphasize ``unified RAG architecture'' more in the writing and remove ``query-free'' from the title.
    \item ``Query-free'' seems to mean ``retriever-free'' here.
    \item Does the proposed architecture still depend on a standalone retriever during training and inference (for passage filtering etc.)? Either way, this is an important modeling condition that should be explicitly mentioned.
\end{enumerate}
}
